3D Scene Inference from Transient Histograms

Time-resolved image sensors that capture light at pico-to-nanosecond timescales were once limited to niche applications but are now rapidly becoming mainstream in consumer devices. We propose low-cost and low-power imaging modalities that capture scene information from minimal time-resolved image sensors with as few as one pixel. The key idea is to flood illuminate large scene patches (or the entire scene) with a pulsed light source and measure the time-resolved reflected light by integrating over the entire illuminated area. The one-dimensional measured temporal waveform, called \emph{transient}, encodes both distances and albedoes at all visible scene points and as such is an aggregate proxy for the scene's 3D geometry. We explore the viability and limitations of the transient waveforms by themselves for recovering scene information, and also when combined with traditional RGB cameras. We show that plane estimation can be performed from a single transient and that using only a few more it is possible to recover a depth map of the whole scene. We also show two proof-of-concept hardware prototypes that demonstrate the feasibility of our approach for compact, mobile, and budget-limited applications.

==> 35_tdh_info.tex <==
\section{Information in a Transient Histogram}\label{sec:tdh-info}
% there is a mix of depth and albedo information
% point to Fig 1 teaser shapes have different tdh shapes
% but there are ambiguities
% how do we recover depths from a single histogram?
% there have been attempts before but it is severely underconstrained
% and ill-posed inverse problem so we need some prior knowledge.
% use MDH!
% unlike MDH, we think of histograms as the primary source of information
% and the RGB provides side information.
% show Fig. 2 here: DNN architecture high level

To get some intuition about what information is contained in a transient histogram, we show some examples for simple shapes in Fig.~\ref{fig:teaser}(b). These transient histograms were captured experimentally; details are discussed later in Section~\ref{subsec:lab-setup}. First, note that the histogram has a sharp leading edge which corresponds to the shortest distance from the sensor to the object. For a simple 2D tilted plane, the transient histogram also has a sharp trailing edge with a drop-off to zero. The support (width of the non-zero region) corresponds to the difference between the farthest and the nearest point on the object. For 3D shapes like the cube and the sphere, there is no sharp trailing edge and the drop-off is more gradual. The 3D ring has a double peak, the distance between these peaks is a function of the angle of the plane of the ring with respect to the sensor.

It is tempting to pose the depth recovery problem as a regularized optimization. Given a measured transient histogram $(\widetilde \varphi_i)_{i=1}^N$,
\[
\underset{z(x,y)}{\mbox{minimize}}\sum_{i=1}^{N} ||\varphi_i - \widetilde\varphi_i|| + R(z)
\]
where the first term forces the measurement to match the theoretical transient histogram $\varphi_i$ in  Eq.~\ref{eq:transient_histogram}, and the second term, $R(z),$ is a regularization term on the depth map. For instance, to force the depth map to be piecewise constant, $R(z)$ can be a total-variation norm. %TODO cite total variation?

Note that the transient histogram has a high temporal resolution, but has no spatial information. So, although the leading edge of a transient histogram gives an accurate estimate of the distance to the nearest point on an object, recovering the depth map $z(x,y)$ from a histogram is severely under-determined even for very simple 2D and 3D shapes. There is no spatial correspondence between $(x,y)$ locations and bin indices $1\leq i\leq N$. So, different physically plausible scenes with different depth maps can produce the same transient histogram.
\begin{myitemize}
  \item {\bf Albedo-depth ambiguity:} The height of a peak conflates albedo and radiometric distance-squared fall-off. A small highly reflective (high albedo) object at a given distance will produce an equally strong peak as a larger but more diffuse (low albedo) one.
  \item {\bf Orientation ambiguity:} The transient histogram is insensitive to chirality; a plane tilted at \SI{45}{\degree} clockwise or counterclockwise with respect to the $x-y$ plane will produce exactly the same transient histogram.
\end{myitemize}
It is therefore not possible to use a standard regularized optimization approach to recover the true depth map from a measured transient histogram.


%\smallskip
%\noindent{\bf Sources of ambiguities:}
%The transient histogram measurement cannot capture chirality: a flat plane
%at a fixed depth tilted $45$ degrees counterclockwise will give the same
%transient histogram as one that is tilted clockwise. Similarly, there is an
%albedo-distance-falloff ambiguity: an object with large albedo can produce a
%stronger peak in the histogram even if it is farther away from the camera than an
%object closer by but with a lower albedo. So there's a very difficult ambiguity
%resolution issue at hand when solving this optimization problem making it
%severely ill-posed.


%\begin{enumerate}
%    \item Definition (how to capture / data acquisition)
%    \item How they differ from GT Histograms (Scene effects / Modeling,
%      Reflectivity, $r^2$ Falloff, Dealing with Pile-up @ Atul)
%    \item Characteristics / Dummy scenes (Simulated scenes maybe with single vs
%      multi-path, real scenes of simple objects)
%    \item Motivation (why use them? cheap, ubiquitous, etc.)
%\end{enumerate}


==> 45_tdh_measurement.tex <==
\section{Measuring a Transient Histogram}\label{sec:tdh-measurement}
% we can measure APD or let's use SPADs! why SPADs? time res, manufacturability
% here we talk about SPAD specific image formation model how r_i translates to
% a histogram measured by a SPAD
% describe the conventinoal image formation, then just say we actually use asynchronous
% async acq - just cite iccv paper.
% later talk about pileup issues, maybe show effect of pileup with simulation
% show a photo of setup that captures it.
The key strength of a transient histogram is its high temporal (depth)
resolution.  Therefore the main requirement to measure a transient histogram is
to use an image sensing technology that is fast enough to capture photons on a
short picosecond-to-nanosecond timescale. A fast avalanche photodiode (APD)
together with a high-sampling-rate analog-to-digital converter (ADC) can be
used to capture the full transient histogram in a single laser pulse. Our
hardware prototype uses a different image sensing technology called
single-photon avalanche diode (SPAD). SPADs have gained popularity in recent
years due to their single-photon sensitivity and extreme time resolution down
to 100s of picoseconds. Moreover, unlike APDs, SPADs can be manufactured at
scale using standard CMOS fabrication technology that used in consumer
electronics such as mobile devices.

Unlike a conventional image sensor that can capture light continuously over the
entire laser period, a SPAD pixel can capture at most one returning photon per
laser period. This is because after each photon detection event, the SPAD pixel
enters a \emph{dead-time} during which the pixel is reset. Conventionally, a
SPAD pixel is operated in synchronization with the pulsed laser; photon
timestamps are acquired over many laser cycles, and a histogram of photon
counts is constructed. We call this the \emph{SPAD histogram}. The scene's
transient histogram can be estimated from a measured SPAD histogram.

\smallskip
\noindent \textbf{Estimating the TH from a SPAD Histogram:}
In each laser cycle, the probability $q_i$ that at least one photon is incident
on the SPAD pixel in bin $i$ can be calculated using Poisson
statistics\footnote{For simplicity, the quantum efficiency of the SPAD pixel
has been absorbed into $\varphi_i$.}: $q_i\!=\!  1\!-\!e^{-\varphi_i}$. The
probability $p_i$ that the SPAD captures a photon in the $i^\text{th}$ bin
follows a geometric distribution: $p_i = q_i \prod_{j<i} q_j$.  For
convenience, the $(N\!+\!1)^\text{st}$ SPAD histogram bin stores the number of
laser cycles with no photon detections: $p_{N+1}=1-\sum_{i=1}^N p_i$. If the
total incident photon flux is low enough such that only a small fraction of the
laser cycles lead to a photon detection, the expected number of photons
measured by the SPAD in bin $1\leq i \leq N$ is proportional to the transient
histogram: $\mathbf{E}[h_i] = L\varphi_i$ where $L$ is the number of laser
cycles. The measured transient histogram is given by: $\widetilde \varphi_i =
\nicefrac{h_i}{L}$.

\begin{figure}[!ht]
\centering \includegraphics[width=0.9\columnwidth]{figures/spad_measure_th.pdf}
\caption{\textbf{Measuring a transient histogram using a SPAD.} (a) The test scene consists of
a ring-shaped target with a background wall. (b) Asynchronous acquisition using
a SPAD reliably captures later photons by avoiding pile-up distortion seen in
conventional acquisition.\label{fig:spad_th_measure}}
\end{figure}

\smallskip
\noindent\textbf{Pile-up:} If the total photon flux incident on the SPAD is
high enough, photon detections in earlier histogram bins prevent later photon
bins from capturing a photon causing pile-up distortions that follow a
characteristic exponentially decaying shape. This pile-up can be due to ambient
light or due to laser photons reflecting from a high albedo target.
Fig.~\ref{fig:spad_th_measure} shows a histogram with and without pileup for
the ring-shaped target with a wall in the background. Observe that the pile-up
distorted histogram has fewer total photon counts in later photon bins. We use
an \emph{asynchronous} acquisition scheme~\cite{gupta_asynchronous_2019} that
counteracts pile-up distortion by operating the SPAD in a free-running mode.
The SPAD pixel enters a dead-time immediately after each photon detection
event, and is reset to capture the next photon after the dead-time period ends.
By capturing raw
timestamps for each photon detection and laser synchronization, photon
timestamps can be re-synchronized to the periodic laser source and a histogram
free from pile-up distortion can be captured.


\begin{figure*}[!ht]
  \includegraphics[width=1.0\textwidth]{figures/teaser.pdf}
  \caption{\textbf{Transient histogram: Measurement and examples.} (a) Measuring a
transient histogram involves illuminating the scene with a pulsed illumination
source such as a pulsed laser which is diffused uniformly over the field of view
of a time-resolved image sensor pixel such as a single-photon avalanche diode.
(b) Some representative examples of different transient histograms obtained with
basic 3D shapes. Observe that the histograms have unique features that capture some
information about the shapes.\label{fig:teaser}}
\end{figure*}

